Instant Graph Neural Networks for Dynamic Graphs

Graph Neural Networks (GNNs) have been widely used for modeling graph-structured data. With the development of numerous GNN variants, recent years have witnessed groundbreaking results in improving the scalability of GNNs to work on static graphs with millions of nodes. However, how to instantly represent continuous changes of large-scale dynamic graphs with GNNs is still an open problem. Existing dynamic GNNs focus on modeling the periodic evolution of graphs, often on a snapshot basis. Such methods suffer from two drawbacks: first, there is a substantial delay for the changes in the graph to be reflected in the graph representations, resulting in losses on the model's accuracy; second, repeatedly calculating the representation matrix on the entire graph in each snapshot is predominantly time-consuming and severely limits the scalability. In this paper, we propose Instant Graph Neural Network (InstantGNN), an incremental computation approach for the graph representation matrix of dynamic graphs. Set to work with dynamic graphs with the edge-arrival model, our method avoids time-consuming, repetitive computations and allows instant updates on the representation and instant predictions. Graphs with dynamic structures and dynamic attributes are both supported. The upper bounds of time complexity of those updates are also provided. Furthermore, our method provides an adaptive training strategy, which guides the model to retrain at moments when it can make the greatest performance gains. We conduct extensive experiments on several real-world and synthetic datasets. Empirical results demonstrate that our model achieves state-of-the-art accuracy while having orders-of-magnitude higher efficiency than existing methods.

==> batch_noexample.tex <==
\section{Batch Update}
\label{sec:batch_update}
We show how to construct estimated vectors for dynamic graphs with one-by-one updated edges in Algorithm~\ref{alg:2}. We adapt our approach in this section to support parallel processing and batch update settings. We begin with an equivalent approach of updating a single node. That is, we can modify the estimate of a node and so avoid repeatedly updating residuals on its neighbors. Taking the insertion of edge $e=(u,v)$ as an example, as described in Section~\ref{sec:instant2structural}, changes in the degrees of nodes $u$ and $v$ have an effect on their neighbors to maintain their equations hold. The primary cause is the transition of $\frac{\bm{\hat{\pi}}(u)}{d(u)^{1-\beta}}$ to $\frac{\bm{\hat{\pi}}(u)}{(d(u)+1)^{1-\beta}}$. As stated in line 5-6 and 9-19 of Algorithm~\ref{alg:2}, we add the increment $\bm{\hat{\pi}}(u)\cdot(\frac{1}{(d(u)+1)^{1-\beta}} - \frac{1}{d(u)^{1-\beta}})$ and $\bm{\hat{\pi}}(v)\cdot(\frac{1}{(d(v)+1)^{1-\beta}} - \frac{1}{d(v)^{1-\beta}})$ to the residuals of each node $w\in N(u)$ and $y\in N(v)$. To avoid modifying all neighbors of nodes $u$ and $v$, we let $\bm{\hat{\pi}}^{\prime}(u) = \bm{\hat{\pi}}(u)\cdot \frac{(d(u)+1)^{1-\beta}}{d(u)^{1-\beta}}$, where $\bm{\hat{\pi}}^{\prime}(u)$ denotes the updated estimate of node $u$. As a result, we have $\frac{\bm{\hat{\pi}}^{\prime}(u)}{(d(u)+1)^{1-\beta}}=\frac{\bm{\hat{\pi}}(u)}{d(u)^{1-\beta}}$, and the equation for node $w\in N(u)$ remains valid. Additionally, the residual of node $u$ needs to be adjusted to account for the change in $\bm{\hat{\pi}}(u)$, i.e., $\Delta \bm{r}(u)=-\frac{\bm{\hat{\pi}}^{\prime}(u)-\bm{\hat{\pi}}(u)}{\alpha}=\bm{\hat{\pi}}^{\prime}(u)\cdot \frac{d(u)^{1-\beta}-(d(u)+1)^{1-\beta}}{\alpha\cdot(d(u)+1)^{1-\beta}}$. Let $\P(w, u)$ be the element of the $w$-th row and $u$-th column of transition matrix $\P$. Note that $\Delta \bm{r}(u) \cdot (1-\alpha)\P(w, u) = \Delta \bm{r}(w)$ (Equation 6), indicating that $\Delta \bm{r}(u)$ can be transformed into $\Delta \bm{r}(w)$ following another push operation. This demonstrates the equivalent nature of these two operations from another perspective. We omit details about updating node $v$ since it is handled similarly. The advantage of modifying $\bm{\hat{\pi}}$ is that we need only update the nodes $u$ and $v$ when edge $e=(u,v)$ arrives, simplifying subsequent parallel processing.

Here we focus on the dynamic propagation algorithm under batch update setting, and Algorithm~\ref{alg:batch_update} gives the pseudo-code. The main idea is to simultaneously calculate the increments caused by multiple edges. Given a set of graph events $M=\{Event_1,\dots,Event_k\}$, line 3 corresponds to the graph updating stage, where the graph in time step $k$, $G_k$, is generated from the initial graph guided by $M$, and $k$ denotes the batch size. Lines 5-9 represent the first step of updating the affected nodes, in which we update the estimates and residuals of these nodes in the way aforementioned. Recall that a portion of an affected node's increment is caused by its added or deleted neighbors. Therefore, we compute the increment by iterating over all new and vanishing neighbors of each affected node, as in lines 10-17. Line 18 invokes the basic propagation algorithm to reduce the error, which is the same as line 7 in Algorithm~\ref{alg:2}.

\begin{algorithm}[t]
% \setlength{\intextsep}{-2mm}
\setlength{\textfloatsep}{2cm}
\setlength{\floatsep}{2cm}
\caption{Parallel Dynamic Propagation Algorithm for Batch Update.}\label{alg:batch_update}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Dynamic graph $\{G_0, M=\{Event_1,\dots,Event_k \}\}$, graph signal vector $\bm{x}$, error threshold $\varepsilon$, teleport probability $\alpha$, convolutional coefficient $\beta$}
\Output{estimated propagation vector $\bm{\hat{\pi}}$,\newline residual vector $\bm{r}$}
$\bm{\hat{\pi}}\leftarrow \bm{0}, \bm{r}\leftarrow\bm{x}$\;
$\bm{\hat{\pi}}, \bm{r}\leftarrow Basic Propagation(G_0, \varepsilon, \alpha, \beta, \bm{\hat{\pi}}, \bm{r})$\;
Generate $G_k$ from updating $G_0$ by $M$\;
% //update graph according to $M$ \\
$V_{_{affected}} \leftarrow \{u|$ the degree of node $u$ has changed$\}$\; 
\textbf{parallel} \For{each $u\in V_{_{affected}}$}
{
  $\Delta d(u) \leftarrow$ the degree to which node $u$ has changed \;
  $\bm{\hat{\pi}}(u) \leftarrow \bm{\hat{\pi}}(u) \cdot \frac{d(u)^{1-\beta}}{(d(u)-\Delta d(u))^{1-\beta}}$ \;
  $\Delta \bm{r}_{_1}(u) \leftarrow \bm{\hat{\pi}}(u) \cdot \frac{(d(u)-\Delta d(u))^{1-\beta} - d(u)^{1-\beta}}{\alpha \cdot d(u)^{1-\beta}} $ \;
  $\bm{r}(u) \leftarrow \bm{r}(u)+\Delta \bm{r}_{_1}(u)$ \;
}
\textbf{parallel} \For{each $u\in V_{_{affected}}$}
{
  $\Delta \bm{r}_{_2}(u) \leftarrow (\bm{\hat{\pi}}(u)\hspace{-0.5mm}+\hspace{-0.5mm}\alpha \bm{r}(u)\hspace{-0.5mm}-\hspace{-0.5mm}\alpha \bm{x}(u)) \hspace{-0.5mm}\cdot\hspace{-0.5mm} \frac{(d(u)-\Delta d(u))^\beta - d(u)^\beta}{d(u)^\beta} $ \;
  \For{each $v \in \{$the added neighbors of node $u\}$}
  {
    $\Delta \bm{r}_{_2}(u) \leftarrow \Delta \bm{r}_{_2}(u) + \frac{(1-\alpha)\bm{\hat{\pi}}(v)}{d(u)^\beta d(v)^{1-\beta}}$ \;
  }
  \For{each $v \in \{$the deleted neighbors of node $u\}$}
  {
    $\Delta \bm{r}_{_2}(u) \leftarrow \Delta \bm{r}_{_2}(u) - \frac{(1-\alpha)\bm{\hat{\pi}}(v)}{d(u)^\beta d(v)^{1-\beta}}$ \;
  }
  $\Delta \bm{r}_{_2}(u) \leftarrow \Delta \bm{r}_{_2}(u) / \alpha $ \;
  $\bm{r}(u) \leftarrow \bm{r}(u)+\Delta \bm{r}_{_2}(u)$ \;
}
$\bm{\hat{\pi}},\bm{r}\leftarrow Basic Propagation(G_k, \varepsilon, \alpha, \beta, \bm{\hat{\pi}}, \bm{r})$\;
return $\bm{\hat{\pi}}$, $\bm{r}$\;
\end{algorithm}
